DoubleEcho: Mitigating Context-Manipulation Attacks in Copresence Verification

Copresence verification based on context can improve usability and strengthen security of many authentication and access control systems. By sensing and comparing their surroundings, two or more devices can tell whether they are copresent and use this information to make access control decisions. To the best of our knowledge, all context-based copresence verification mechanisms to date are susceptible to context-manipulation attacks. In such attacks, a distributed adversary replicates the same context at the (different) locations of the victim devices, and induces them to believe that they are copresent. In this paper we propose DoubleEcho, a context-based copresence verification technique that leverages acoustic Room Impulse Response (RIR) to mitigate context-manipulation attacks. In DoubleEcho, one device emits a wide-band audible chirp and all participating devices record reflections of the chirp from the surrounding environment. Since RIR is, by its very nature, dependent on the physical surroundings, it constitutes a unique location signature that is hard for an adversary to replicate. We evaluate DoubleEcho by collecting RIR data with various mobile devices and in a range of different locations. We show that DoubleEcho mitigates context-manipulation attacks whereas all other approaches to date are entirely vulnerable to such attacks. DoubleEcho detects copresence (or lack thereof) in roughly 2 seconds and works on commodity devices.

==> rprox.tex <==
\section{\our}
\label{sec:rprox}
\our{} uses audio as the context to verify copresence of two devices and leverages RIR to mitigate context-manipulation attacks. We focus on audio for two main reasons. First, sensors to capture audio signals (i.e., microphones) are widely available on commodity devices. Second, an audio signal is heavily affected by the surrounding space; thus, acoustic RIR may allow to tell whether two devices are within the same room.


Further, \our{} accommodates scenarios where the entropy of context data is insufficient (e.g., a silent room), by \emph{injecting} a stimulus (i.e., a chirp signal) in the environment. Therefore, we assume prover and verifier to be equipped with microphones and at least one of them to be equipped with a speaker.


%\begin{figure}[htpb]
%\begin{center}
%\fbox{%
%\procedure[linenumbering]{\textbf{DoubleEcho}(\sound{},\prover{},\verifier{}, $r_P$, $r_V$, \textrm{Classify()}) }{%
%\text{Emit } \sound{}  \text{ in room spaces } r_P, r_V \\
%\text{Record }\sound_P \gets \sound \circledast r_P, \sound_V \gets \sound \circledast r_V \\
%h_P \gets \sound_P/\sound; h_V \gets \sound_V / \sound \\
%\hat{\gt} \gets \textrm{Classify}(||h_P - h_V||) \\
%\pcreturn \hat{\gt}
%}
%}
%\end{center}
%\caption{RIR based \cov{}.}
%\label{fig:doubleecho}
%\end{figure}


\cla{I would substitute the picture with one that shows how the protocol works along the lines of figure  2.}
Fig.~\ref{fig:doubleecho} illustrates the \our{} approach at high level between a prover device \prover{} and a verifier device \verifier{}. We assume that \prover{} and \verifier{} have access to an authenticated channel (i.e., share a secret key). The following steps are executed.

\begin{enumerate}
\item \textbf{Start.} The protocol may be triggered by either the prover or the verifier. This is done by sending a well-known message over the authenticated channel. During this stage, the verifier also sends a random nonce to the prover.~\footnote{The nonce is used as a challenge to prevent replay attacks.}
\item \textbf{Playing and Recording.} The device with a speaker (without loss of generality we assume \verifier{} has a speaker) plays a known audio clip \sound; at the same time both devices record audio in the environment via their microphones.
\item \textbf{RIR.} The verifier (resp. the prover) extract the RIR $h_{\verifier}$ (resp. $h_{\prover}$) based on the original audio clip \sound{} (the system's input) and the signal recorded via its microphone (the system's output). The prover sends its RIR $h_{\prover}$ to the verifier via the authenticated channel, along with the nonce received previously from the verifier.
\item \textbf{Comparison.} The verifier compares the nonce sent at the beginning of the protocol with the one received from the prover. If the two nonces are different, the verifier assumes a replay attack and aborts. Otherwise, the verifier compares $h_\verifier$ computed locally with $h_\prover$ received by the prover to decide whether the two devices are copresent or not.
\end{enumerate}



\subsection{RIR Comparison}

During the last step of the protocol, the verifier compares its RIR with the one computed by the prover. The comparison mechanism clearly has a dramatic impact on the performance of the system in terms of usability and security. That is, the comparison function should enable the verifier to reliably detect scenarios where the prover is copresent as well as scenarios where the prover is far away. Previous work~\cite{DBLP:conf/esorics/HaleviMSX12} proposes to use basic functions like cross-correlation between the two signals in the time domain; hence the verifier considers the prover to be copresent if the cross-correlation is above a given threshold. We did not obtain decent results with cross-correlation. Other ways to compare RIR signals based on Power Spectral Density (PSD), Mel Frequency Cepstral, Linear Predictive Coding~\cite{Rossi2013} or Reverberation Time of wide band signals, did not bring us good results either.

We therefore opted for a binary classifier based on features extracted from RIR. We used the feature described in Section~\ref{sec:background:features}. The next section provides more details about the classifier and how we selected relevant features for copresence verification.






